LOCATE: Self-supervised Object Discovery via Flow-guided Graph-cut and Bootstrapped Self-training

Learning object segmentation in image and video datasets without human supervision is a challenging problem. Humans easily identify moving salient objects in videos using the gestalt principle of common fate, which suggests that what moves together belongs together. Building upon this idea, we propose a self-supervised object discovery approach that leverages motion and appearance information to produce high-quality object segmentation masks. Specifically, we redesign the traditional graph cut on images to include motion information in a linear combination with appearance information to produce edge weights. Remarkably, this step produces object segmentation masks comparable to the current state-of-the-art on multiple benchmarks. To further improve performance, we bootstrap a segmentation network trained on these preliminary masks as pseudo-ground truths to learn from its own outputs via self-training. We demonstrate the effectiveness of our approach, named LOCATE, on multiple standard video object segmentation, image saliency detection, and object segmentation benchmarks, achieving results on par with and, in many cases surpassing state-of-the-art methods. We also demonstrate the transferability of our approach to novel domains through a qualitative study on in-the-wild images. Additionally, we present extensive ablation analysis to support our design choices and highlight the contribution of each component of our proposed method.

==> 06_extras.tex <==

\begin{table}
\centering
\begin{tabular}{|l|c|c|}
\hline
\textbf{Dataset}  & \textbf{w/o self-loops}($\mathcal{J}~\uparrow$) & \textbf{w/ self-loops}($\mathcal{J}~\uparrow$) \\ 
\hline
DAVIS16 & 78.00 & \textbf{78.03}  \\
\hline
SegTrackv2 & 68.28 & \textbf{76.27} \\
\hline
FBMS59 & \textbf{63.93} & 63.69 \\
\hline
\end{tabular}
\caption{\textbf{Ablation on self-loops in the adjacency matrix $W$ for graph-cut}. Overall we observe comparable performance with and without self-loops in the adjacency matrix. $W_{ii} = 0$}
\label{tab:self_loop_ablations}
\end{table}



\begin{table}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{\# training iterations} & \textbf{10k} & \textbf{15k} & \textbf{20k} \\ 
\hline
\textbf{DAVIS16}($\mathcal{J}~\uparrow$) & 77.73 & 78.48 & \textbf{78.98}\\
\hline
\end{tabular}
\caption{\textbf{Ablation on the number of training iterations of the segmentation network}. We train the segmentation network for 20k iterations hereon, unless stated otherwise.}
\label{tab:training_iterations}
\end{table}



\begin{table}
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Iteration (Model Initialization)} & \textbf{DAVIS16}($\mathcal{J}~\uparrow$) \\ 
\hline
Iteration 1 (N/A)  & 78.98 \\
\hline 
Iteration 2 (model initialized from iteration 1) &  \\
\hline
Iteration 2 (model training from scratch) & 79.91 \\
\hline
\end{tabular}
\caption{\textbf{Ablation on the model initialization during self-distillation}. TODO cite BLIP if from-scratch training works better.}
\label{tab:model_init_ablation}
\end{table}




\begin{table}
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Seed}  & \textbf{DAVIS16}($\mathcal{J}~\uparrow$) \\ 
\hline
42 & 78.98  \\
\hline
332 & 78.64 \\
\hline
597 & 78.12 \\
\hline
720 & 78.17 \\
\hline
446 & 79.10 \\
\hline
\hline
mean $\pm$ std dev. & 78.6 $\pm$ 0.45 \\
% \hline
% taking mean of sigmoid outputs from all the models & 78.9 \\
\hline
ensemble (majority voting) & 78.82 \\
\hline
\end{tabular}
\caption{\textbf{Ensemble with different seeds}. We distill using graph-cut masks as pseudo ground-truths with 5 different seeds to create an ensemble. All models are trained for 20k iterations.}
\label{tab:ensemble_ablations}
\end{table}



\begin{table}
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Bootstrapping w/ ensembles}  & \textbf{DAVIS16}($\mathcal{J}~\uparrow$) \\ 
\hline
Iteration 0 (graph-cut masks) & 78.03 \\ 
\hline
Iteration 1 (ensemble) & 78.82 \\
\hline
Iteration 2 & 78.66 \\
\hline
% Iteration 3 &  \\
% \hline
\end{tabular}
\caption{\textbf{Bootstrapping w/ ensembles}. We create an ensemble of 5 segmentation networks and bootstrap the training process with ensemble outputs.}
\label{tab:bootstrapping_with_ensembles}
\end{table}


\begin{table}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Eval Setup} & \textbf{DAVIS16($\mathcal{J}~\uparrow$)} & \textbf{SegTrackv2($\mathcal{J}~\uparrow$)} & \textbf{FBMS59($\mathcal{J}~\uparrow$)} \\ 
\hline
\hline
\textbf{(a) Zero-shot} & - & 65.56~(iter~4) & 67.83~(iter~7)\\
\hline
\textbf{(b) Excess data}  & 80.24 & 81.07 & 66.43 \\
\hline
\end{tabular}
\caption{\textbf{(a) Zero-shot evaluation.} A segmentation network trained only on the DAVIS16 dataset is evaluated on the SegTrackv2 and FBMS59 datasets. (frame avg is reported).\\ \textbf{(b) Learning with excess data.} A segmentation network trained on all the videos combined is evaluated on each individual dataset. The network is trained for a total of 80k iterations with checkpoints every 5k iterations. Best scores are reported for each dataset.}
\label{tab:transfer_learning_VOS}
\end{table}



\subsection{Discussion on the key features/advantages of our approach}
\begin{itemize}
    \item simple \& effective pipeline
    \item completely unsupervised (ARFlow + iterative self-training)
    \item no (significant) post-processing techniques used \& no Test-time adaptation making our method applicable in real applications (post-processing takes up lot of time)
    \item trained on videos -> but can be applied to still images as well; can be easily extended to image saliency detection tasks
    \item does not require optical flow as input at the time of inference
    \item learning-free graph-cut step
    \item our approach is not very sensitive to the choice of optical flow estimation model; the current SOTA- Guess What Moves, on the other hand, suffers a significant drop in the mIoU score from 79.5 to 66.9 by changing the flow estimation model from RAFT to ARFlow.
    \item Our end-to-end approach of flow-guided graph-cut followed by self-training is generalizable across datasets- even those for which ground truth annotation is not available, for e.g., in FBMS59 dataset only $\sim$720 out of 13k images have ground truth annotations. (to address the question: Why not just use ground-truth annotations to train the segmentation network, $\phi$?)
    
\end{itemize}
